Multi-characteristic Subject Selection from Biased Datasets

Subject selection plays a critical role in experimental studies, especially ones with human subjects. Anecdotal evidence suggests that many such studies, done at or near university campus settings suffer from selection bias, i.e., the too-many-college-kids-as-subjects problem. Unfortunately, traditional sampling techniques, when applied over biased data, will typically return biased results. In this paper, we tackle the problem of multi-characteristic subject selection from biased datasets. We present a constrained optimization-based method that finds the best possible sampling fractions for the different population subgroups, based on the desired sampling fractions provided by the researcher running the subject selection.We perform an extensive experimental study, using a variety of real datasets. Our results show that our proposed method outperforms the baselines for all problem variations by up to 90%.

==> 2-fig_tex/biased_data.tex <==
\begin{figure*}[h!]

\centering %
  \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\linewidth]{4-figures/initial_kloan.pdf}
    \caption{joint initial dist. for Kaggle Loan Data} 
    \label{fig:kloan_initial} 
  \end{subfigure}\hfil % 
  \begin{subfigure}[b]{0.30\textwidth}
    \includegraphics[width=\linewidth]{4-figures/initial_github.pdf}
    \caption{joint initial dist. for Github Loan Data} 
    \label{fig:github_initial} 
 \end{subfigure}\hfil % 
  \begin{subfigure}[b]{0.30\textwidth}
    \includegraphics[width=\linewidth]{4-figures/initial_titanic.pdf}
    \caption{joint initial dist. for Kaggle Titanic Data} 
    \label{fig:titanic_initial} 
  \end{subfigure}
  
\caption{joint initial distributions for Kaggle loan, Github loan and kaggle titanic biased datasets}

\label{fig:biased_data}   
\end{figure*} 

==> 2-fig_tex/initial_github_loan.tex <==
\begin{figure}[!ht]
  \centering
  \includegraphics[width=1\linewidth]{4-figures/initial_github.png}
  \caption{joint initial distribution for Github Loan Data}
  \label{fig:github_initial}
\end{figure}

==> 2-fig_tex/initial_kaggle_titanic.tex <==
\begin{figure}[!ht]
  \centering
  \includegraphics[width=1\linewidth]{4-figures/initial_tiatanic.png}
  \caption{joint initial distribution for Kaggle Titanic Data}
  \label{fig:titanic_initial}
\end{figure}

==> 2-fig_tex/oneVar_results.tex <==
\begin{figure}[!ht]
  \centering
  \includegraphics[height=3.1cm, width=0.5\linewidth]{4-figures/oneVariable_results.pdf}
  \caption{comparison of cosine distance obtained by baselines (PSRS, OSRS, RA \&\ WRS) and optimization-based (OP) method using Kaggle Titanic data with only one characteristic}
 %\vspace{-0.5cm}
  \label{fig:oneVar_results}
\end{figure}

==> 2-fig_tex/pitt_fixed_range.tex <==
\begin{figure}[ht!]
  \centering
  \includegraphics[height=3.2cm, width=0.5\linewidth]{4-figures/pitt_fixed_range_results.pdf}
  %\caption{comparison of cosine distance for fixed and range-based variations obtained by baselines (RA = Rank Aggregation, %WRS = Weighted Random Sampling) and optimization-based (OP) method using survey data with ideal distribution from %Pittsburgh census}
  \caption{comparison of cosine distance for fixed and range-based variations obtained by baselines and optimization-based (OP) method for survey data with ideal distribution from Pittsburgh census.}
  %\vspace{-0.5cm}
  \label{fig:pitt_fixed_range}
\end{figure}

==> 3-table_tex/joint_ideal_eaxmple.tex <==
\begin{table}[h!]
\small
\setlength{\tabcolsep}{2pt}
\centering
\caption{an example of calculation of joint ideal percentage by algorithm \ref{alg:jointideal}, based on the age and gender distributions collected from the Pittsburgh census reporter}
\label{tab:ji_example}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\diagbox[width=10em]{\textbf{gender groups}}{\textbf{age groups}} & \textbf{\begin{tabular}[c]{@{}c@{}}20-\\ (20\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}20s\\ (23\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}30s\\ (16\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}40s\\ (9\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}50s\\ (11\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}60s\\ (12\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}70+\\ (9\%)\end{tabular}} \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}male\\ (48\%)\end{tabular}} & 9.6\% & 11.04\% & 7.68\% & 4.32\% & 5.28\% & 5.76\% & 4.32\% \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}female\\ (52\%)\end{tabular}} & 10.4\% & 11.96\% & 8.32\% & 4.68\% & 5.72\% & 6.24\% & 4.68\% \\ \hline
\end{tabular}
\end{table}


